On the Security Blind Spots of Software Composition Analysis

Modern software heavily relies on the use of components. Those components are usually published in central repositories, and managed by build systems via dependencies. Due to issues around vulnerabilities, licenses and the propagation of bugs, the study of those dependencies is of utmost importance, and numerous software composition analysis tools have emerged for this purpose. A particular challenge are hidden dependencies that are the result of cloning or shading where code from a component is "inlined", and, in the case of shading, moved to different namespaces. We present a novel approach to detect vulnerable clones in the Maven repository. Our approach is lightweight in that it does not require the creation and maintenance of a custom index. Starting with 29 vulnerabilities with assigned CVEs and proof-of-vulnerability projects, we retrieve over 53k potential vulnerable clones from Maven Central. After running our analysis on this set, we detect 727 confirmed vulnerable clones (86 if versions are aggregated) and synthesize a testable proof-of-vulnerability project for each of those. We demonstrate that existing SCA tools often miss those exposures. At the time of submission those results have led to changes to the entries for six CVEs in the GitHub Security Advisory Database (GHSA) via accepted pull requests, with more pending.

==> pipeline-results.tex <==
\begin{table*}
	\begin{tabular}{|l|p{2cm}p{2cm}p{2cm}p{2cm}p{2cm}p{2cm}|}
	\hline
	vulnerability&query results&consolidated&no dependency&clones detected&pov compiled&pov tested \\
	\hline
	CVE-2015-6420&1,250 (87)&1,196 (82)&982 (66)&553 (20)&549 (20)&3 (3) \\
	CVE-2016-2510&408 (83)&401 (80)&390 (79)&12 (4)&12 (4)&3 (2) \\
	CVE-2018-10237&3,285 (384)&2,077 (285)&1,009 (181)&177 (36)&177 (36)&22 (6) \\
	CVE-2021-44228&1,137 (92)&1,064 (79)&339 (33)&185 (7)&182 (7)&15 (3) \\
	CVE-2022-25845&1,532 (151)&1,358 (130)&419 (58)&116 (17)&115 (17)&30 (6) \\
	CVE-2022-38749&2,217 (185)&1,076 (115)&585 (79)&39 (10)&29 (8)&20 (5) \\
	CVE-2022-42889&2,256 (152)&1,236 (80)&339 (34)&92 (8)&92 (8)&4 (1) \\
	CVE-2022-45688&4,160 (347)&1,802 (117)&1,333 (94)&648 (41)&579 (24)&457 (23) \\
	\hline
	(sum)&16,245 (1,481)&10,210 (968)&5,396 (624)&1,822 (143)&1,735 (124)&554 (49) \\
	\hline
	\end{tabular}
	\caption{\label{tab:pipeline}Processed Artifacts at each stage, numbers in brackets are classes of artifacts with the same group and artifact id (i.e., versions are ignored)}
\end{table*}


==> sca-results.tex <==
We set out to identify vulnerabilities in artifacts missed by existing tools. Table~\ref{tab:scacve} lists if each CVE is detected by the SCA tools. Table~\ref{tab:scaresults} lists the proportion of artifacts that SCA tools report as vulnerable. 

%Notably, \emph{steady} and \emph{grype} report the  vulnerable dependency in \textit{com.google.guava}, and \emph{steady} also reports them for \textit{com.guicedee.services}.

%Those results support our claim that our methods reveals vulnerable artifacts missed by existing SCA tools.
  
Not surprisingly, \textit{steady} performs better than purely dependency-based tools as it employs program analysis. However, this is not consistent. The fact that is performs poorly on newer vulnerabilities suggests that updates of the database it relies on (project KB~\footnote{\url{https://sap.github.io/project-kb/}}~\cite{ponta2019msr}) are lagging behind. 

More surprisingly, \textit{owasp} also outperforms other tools for several CVEs. This is interesting as it  relies on metadata, and (unlike \textit{steady}) does not perform code analysis.  However, it also analyses runtime metadata (as opposed to buildtime metadata, i.e. poms) located in the deployed artifacts (jars), usually in \texttt{META-INF} and its subfolders. This enables it to infer dependencies tools only relying on poms might miss. 

%For instance, poms often use variables (properties) to reference dependencies or parent poms. In the metadata within jars, those variables are resolved, and therefore enable a more accurate dependency analysis

% this results disappeared after rerun:
%A closer analysis of some of the results yields further surprises. \textit{Snyk} does report CVE-2022-38749 in one of the artifacts we detect (\textit{com.alipay.sofa.acts:acts-common-util:1.0.0}). However, this is a false true positive -- the provenance data in the \textit{snyk} report suggests that this is based on an alternative transitive dependency on \textit{snakeyaml} via \textit{testNG}, used for testing by the respective project.


\begin{table}


\begin{tabular}{|l|rrrr|}
\hline
vulnerability & grype & owasp & snyk & steady \\
\hline
CVE-2015-6420 & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\times$ \\
CVE-2016-2510 & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ \\
CVE-2018-10237 & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ \\
CVE-2021-44228 & $\checkmark$ & $\checkmark$ & $\checkmark$& $\checkmark$ \\
CVE-2022-25845 & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\times$ \\
CVE-2022-38749 & $\checkmark$ & $\checkmark$ & $\checkmark$ &  $\times$ \\
CVE-2022-42889 & $\checkmark$ & $\checkmark$ & $\checkmark$ &  $\times$ \\
CVE-2022-45688 & $\checkmark$ & $\checkmark$ & $\checkmark$ &  $\times$ \\
\hline
\end{tabular}
\caption{\label{tab:scacve}Vulnerability detection by SCA tool for evaluation artifacts}

\end{table}




\begin{table}

\begin{tabular}{|l|r|rrrr|}
\hline
vulnerability & (sum) & grype & owasp & snyk & steady \\
\hline
CVE-2015-6420 & 3 & 0 & 0 & 0 & 0 \\
CVE-2016-2510 & 3 & 0 & 1 & 1 & 3 \\
CVE-2018-10237 & 22 & 8 & 12 & 0 & 17 \\
CVE-2021-44228 & 15 & 0 & 14 & 0 & 15 \\
CVE-2022-25845 & 30 & 0 & 2 & 0 & 0 \\
CVE-2022-38749 & 20 & 0 & 20 & 0 & 0 \\
CVE-2022-42889 & 4 & 0 & 4 & 0 & 0 \\
CVE-2022-45688 & 454 & 0 & 33 & 0 & 0 \\
\hline
\textbf{(sum)} & \textbf{554} & \textbf{8} & \textbf{86}  & \textbf{1} & \textbf{35} \\

\hline
\end{tabular}
\caption{\label{tab:scaresults}Total of artifacts reported by each SCA tool from  the set of vulnerable artifacts by CVE}

\end{table}




%\todo[inline] {Results go here, perhaps a short summary is enough unless we  find something really interesting. We should also report that the tools do pick up the CVEs in xshady}.

==> vulnerable-artifacts.tex <==
\begin{table*}
	\begin{tabular}{|lll|}
	\hline
	groupId:versionId&versions&shaded \\
	\hline
	\multicolumn{3}{|c|}{CVE-2015-6420} \\
	\hline
	net.\-sourceforge.\-collections:\-collections-generic&1&yes \\
	org.\-apache.\-servicemix.\-bundles:\-org.\-apache.\-servicemix.\-bundles.\-collections-generic&1&yes \\
	org.\-apache.\-servicemix.\-bundles:\-org.\-apache.\-servicemix.\-bundles.\-commons-collections&1&no \\
	\hline
	\multicolumn{3}{|c|}{CVE-2016-2510} \\
	\hline
	<masked-artifact-1>&2&no \\
	org.\-beanshell:\-bsh&1&no \\
	\hline
	\multicolumn{3}{|c|}{CVE-2018-10237} \\
	\hline
	com.\-google.\-guava:\-guava-jdk5&8&no \\
	com.\-googlecode.\-guava-osgi:\-guava-osgi&2&no \\
	de.\-mhus.\-ports:\-vaadin-shared-deps&5&yes \\
	org.\-apache.\-servicemix.\-bundles:\-org.\-apache.\-servicemix.\-bundles.\-guava&4&no \\
	org.\-hudsonci.\-lib.\-guava:\-guava&2&no \\
	org.\-sonatype.\-sisu:\-sisu-guava&1&no \\
	\hline
	\multicolumn{3}{|c|}{CVE-2021-44228} \\
	\hline
	com.\-guicedee.\-services:\-log4j-core&13&no \\
	org.\-xbib.\-elasticsearch:\-log4j&1&no \\
	uk.\-co.\-nichesolutions.\-logging.\-log4j:\-log4j-core&1&no \\
	\hline
	\multicolumn{3}{|c|}{CVE-2022-25845} \\
	\hline
	com.\-rover12421:\-fastjson&1&no \\
	com.\-taobao.\-arthas:\-fastjson&1&no \\
	com.\-weicoder.\-extend:\-fastjson-extend&1&no \\
	com.\-weicoder.\-extend:\-json-extend&2&no \\
	com.\-weicoder.\-fork:\-fastjson-jdk11&1&no \\
	org.\-apache.\-servicemix.\-bundles:\-org.\-apache.\-servicemix.\-bundles.\-fastjson&24&no \\
	\hline
	\multicolumn{3}{|c|}{CVE-2022-38749} \\
	\hline
	be.\-cylab:\-snakeyaml&1&no \\
	<masked-artifact-2>&1&no \\
	<masked-artifact-3>&4&no \\
	org.\-testifyproject.\-external:\-external-snakeyaml&11&yes \\
	pl.\-droidsonroids.\-yaml:\-snakeyaml&3&no \\
	\hline
	\multicolumn{3}{|c|}{CVE-2022-42889} \\
	\hline
	com.\-guicedee.\-services:\-commons-text&4&no \\
	\hline
	\multicolumn{3}{|c|}{CVE-2022-45688} \\
	\hline
	com.\-dimajix.\-flowman:\-flowman-plugin-json&29&yes \\
	com.\-github.\-anandvarkeyphilips:\-json-java-ordered&1&no \\
	com.\-github.\-fangjinuo.\-easyjson:\-orgjson-to-easyjson&23&no \\
	com.\-github.\-jinahya:\-json-retrotranslated&1&no \\
	com.\-github.\-tsohr:\-json&1&yes \\
	com.\-guicedee.\-services:\-json&241&no \\
	com.\-jeramtough:\-jtlog&6&yes \\
	com.\-jwebmp.\-jre11:\-json&3&no \\
	com.\-jwebmp.\-thirdparty:\-json&6&no \\
	com.\-jwebmp:\-json&9&no \\
	com.\-xliic:\-json-java&1&no \\
	in.\-co.\-s13:\-common-json&2&no \\
	io.\-github.\-bes2008.\-solution.\-easyjson:\-orgjson-to-easyjson&5&no \\
	<masked-artifact-4>&7&yes \\
	io.\-gravitee.\-policy:\-gravitee-policy-mock&5&yes \\
	io.\-gravitee.\-policy:\-gravitee-policy-xml-json&5&yes \\
	<masked-artifact-5>&18&no \\
	org.\-codeartisans:\-org.\-json&1&no \\
	org.\-graalvm.\-tools:\-coverage&22&yes \\
	org.\-graalvm.\-tools:\-dap&22&yes \\
	org.\-graalvm.\-tools:\-lsp&22&yes \\
	org.\-graalvm.\-tools:\-profiler&22&yes \\
	org.\-graalvm.\-tools:\-warmup&5&yes \\
	\hline
	\end{tabular}
	\caption{\label{tab:vulnerableartifacts}Artifacts with Vulnerable Components Detected}
\end{table*}

